Certified Adversarial Robustness for Deep Reinforcement Learning

Deep Neural Network-based systems are now the state-of-the-art in many robotics tasks, but their application in safety-critical domains remains dangerous without formal guarantees on network robustness. Small perturbations to sensor inputs (from noise or adversarial examples) are often enough to change network-based decisions, which was already shown to cause an autonomous vehicle to swerve into oncoming traffic. In light of these dangers, numerous algorithms have been developed as defensive mechanisms from these adversarial inputs, some of which provide formal robustness guarantees or certificates. This work leverages research on certified adversarial robustness to develop an online certified defense for deep reinforcement learning algorithms. The proposed defense computes guaranteed lower bounds on state-action values during execution to identify and choose the optimal action under a worst-case deviation in input space due to possible adversaries or noise. The approach is demonstrated on a Deep Q-Network policy and is shown to increase robustness to noise and adversaries in pedestrian collision avoidance scenarios and a classic control task.

==> discussion.tex <==

%!TEX root = main.tex

\section{Discussion and Future Work} \label{sec:discussion}
\subsection{Accurately calibrated model uncertainty estimates}
In another novel scenario, an agent was trained to avoid collaborative RVO agents and tested on uncollaborative agents. The uncertainty values did not significantly increase, which can be explained by two reasons. First, uncollaborative agents could not be seen as novel for the model; possibly, because RVO agents, further away from the agent also act in a straight line. The fact that humans think that uncollaborative agents might be novel for a model that has only been trained on collaborative agents, does not change the fact that the model might be generalizable enough to not see it as novel. Another explanation is the observed overconfidence of dropout as an uncertainty estimate. Future work will find unrevealed estimates of model uncertainty for neural networks that provide stronger guarantees on the true model uncertainty. 
%\begin{figure}[t]
%  \centering
%    \includegraphics [trim=0 0 0 0, clip, angle=0, width=1.0\columnwidth,
%  keepaspectratio]{figures/static_obst_straight_line_unc_2_fused}
%  \caption{Sparse training data. A model was trained and tested to predict collision labels with an obstacle in the middle. The amount of training data was increased from the left to the right plot. The model uncertainty (y-axis) identifies regions where training samples are sparse and exact decision boundaries (green/red) unexplored.\blXX{should I even put this?}}
%  \label{fig:explain_away_unc} 
%    \centering
%  \vspace{-.1in}
%\end{figure}
%\subsection{Model uncertainty for detection of sparse training data}
%Apart from using uncertainty for regionally detecting novel observations, uncertainty could also be used to avoid unsafe regions of sparse training data. ~\Cref{fig:explain_away_unc} shows how uncertainty is high in the unexplored label transition regions and decreases over training time. Similar to~\cref{fig:out_of_dist}, a network was trained to predict collision (red) and no-collision (green) labels with an obstacle in the middle. The model is tested with the same obstacle, after having experienced increasing amounts of training data. With few data the model gives uncertain collision predictions at the decision boundaries (left plot). As we increase the dataset size, the model explores the intersection regions and gets more confident (right plot). In a case of sparse training samples, our controller would take a more certainly safe action away from the decision boundary and drive a safer policy than an uncertainty-unaware controller.
